PMC-CLIP: Contrastive Language-Image Pre-training using Biomedical Documents

Foundation models trained on large-scale dataset gain a recent surge in CV and NLP. In contrast, development in biomedical domain lags far behind due to data scarcity. To address this issue, we build and release PMC-OA, a biomedical dataset with 1.6M image-caption pairs collected from PubMedCentral's OpenAccess subset, which is 8 times larger than before. PMC-OA covers diverse modalities or diseases, with majority of the image-caption samples aligned at finer-grained level, i.e., subfigure and subcaption. While pretraining a CLIP-style model on PMC-OA, our model named PMC-CLIP achieves state-of-the-art results on various downstream tasks, including image-text retrieval on ROCO, MedMNIST image classification, Medical VQA, i.e. +8.1% R@10 on image-text retrieval, +3.9% accuracy on image classification.

==> content/DatasetOverview.tex <==
\section{Dataset Overview}
\label{sec:dataset_overview}
% Larger: 1.6M
% Diversity: various modality, disease, body parts
% Fairness
%   - Age and Gender
%   - Quality, Novalty
%   - no privacy issue: collected from published scientific papers
In this section, we will give a brief overview of our dataset.
The [PMC OA] dataset contains 1.8 million samples spanning a wide range of diagnostic procedures and disease. We also balance the patients' age and gender to avoid bias.

\noindent \textbf{Diagnostic Procedure} is used to determine the nature or identity of a disease or disorder.
As shown in Figure \ref{fig:diagnostic}
Common modalities appears a lot in \dataset{}, e.g. X-ray, MRI, Ultrasound.
And some relatively fewer modalities are also covered (e.g. radioisotope scan, fluorescence imaging).

% \noindent \textbf{Symptom}

\noindent \textbf{Disease and finding} are given in free-form text, allowing for elaborate identification and analysis. For instance, eye diseases can be further categorized into Cataracts, Conjunctivitis, Macular degeneration, fish eye disease, etc.
Figure \ref{fig:disease} illustrate the frequently used words in diagnosis.

\noindent Apart from the large scope of [PMC OA], we consider fairness issues.
The sex-ratio across ages is shown in Figure \ref{fig:ages}.
The dataset is approximately gender-balanced, with 54\% males.


\begin{figure*}[htpb]
    \centering
    \subfigure[Diagnostic Procedure]{
        % \begin{minipage}[t]{0.5\linewidth}
		% \centering
		\includegraphics[height=1.2in]{content/fig/data_overview/diagnostic_procedure.png}
        % \caption{Diagnostic Procedure}
        \label{fig:diagnostic}
		% \end{minipage}
    }
    \subfigure[Disease]{
        % \begin{minipage}[t]{0.5\linewidth}
		% \centering
		\includegraphics[height=1.2in]{content/fig/data_overview/disease.png}
        \label{fig:disease}
		% \end{minipage}
    }
    \subfigure[Ages]{
        % \begin{minipage}[t]{0.5\linewidth}
		% \centering
		\includegraphics[height=1.2in]{content/fig/data_overview/ages.png}
        \label{fig:ages}
		% \end{minipage}
    }
    \label{fig:dataset_overview}
    \caption{Dataset Overview}
\end{figure*}



% \begin{table*}[htpb]
%     \centering
%     \setlength{\tabcolsep}{6pt} % Default value: 6pt
%     % \renewcommand{\arraystretch}{1.5} % Default value: 1
%     \begin{tabular}{l|c|l}
%         Dataset & Data Size & Data Type \\
%         \toprule
%         ROCO & 81K & Radiology \\
%         MedICaT & 200K & Radiology and Charts \\
%         Ours & 1.6M & Radiology, Microscopy, Ultrasound, etc. \\
%         \midrule
%     \end{tabular}
%     \caption{Dataset Comparison
%     \weixiong{better show this more directly with figures}
%     }
%     \label{tab:dataset}
% \end{table*}


==> content/tab/classification_1.tex <==
% 1. 在同样的 data 上 MedCLIP 超过 SOTA, 并且加上 PMC_OA 之后效果进一步提升
% 1. 这里 MedMNIST Benchmark 测了很多方法(Res18, Res50, Google AutoML Vision), 但是表格只记录最高的
\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{6pt} % Default value: 6pt
    % \renewcommand{\arraystretch}{1.5} % Default value: 1
    \begin{tabular}{c|ccc|ccc|ccc}
        Dataset & \multicolumn{3}{c|}{PneumoniaMNIST} & \multicolumn{3}{c|}{BreastMNIST} & \multicolumn{3}{c}{DermaMNIST} \\
        Methods & AUC$\uparrow$ & ACC$\uparrow$ & F1$\uparrow$ & AUC$\uparrow$ & ACC$\uparrow$ & F1$\uparrow$ & AUC$\uparrow$ & ACC$\uparrow$ & F1$\uparrow$ \\ \toprule
        MedMNIST Benchmark & \textbf{99.10} & 94.60 & ~ & 91.90 & 86.30 & ~ & 92.00 & 76.80 & ~\\
        DWT-CV \cite{cheng2022dwt} & 95.69 & 88.67 & ~ & 89.77 & 85.68  & ~ & 91.67 & 74.75  & ~ \\ 
        SADAE \cite{ge2022self} & 98.30 & 91.80 & ~ & 91.50 & 87.80 & ~ & 92.70 & 75.90 & ~\\
        \midrule
        ROCO(LinearProbe) & 89.20 & 81.57 & ~ & 78.85 & 71.47 & ~ & 87.28 & 64.69 & ~\\
        Ours(LinearProbe) & 93.35 & 85.50 & ~ & 88.41 & 79.49 & ~ & 90.81 & 71.97 & ~\\
        \midrule
        ROCO(Finetune) & 98.78 & 93.99 & ~ & 94.42 & 90.06 & ~ & 91.11 & 78.65 & ~\\
        Ours(Finetune) & 99.02 & \textbf{95.35} & ~ & \textbf{94.56} & \textbf{91.35} & ~ & \textbf{93.41} & \textbf{79.80} & ~\\
        \midrule
    \end{tabular}
    \caption{MedMNIST}
    \label{tab:MedMNIST}
\end{table*}


% =============================================================================
% 
% \begin{table*}[htpb]
%     \centering
%     \setlength{\tabcolsep}{6pt} % Default value: 6pt
%     % \renewcommand{\arraystretch}{1.5} % Default value: 1
%     \begin{tabular}{l|cc|cc|cc}
%         \multirow{2}{*}{Methods}  & \multicolumn{2}{c|}{PneumoniaMNIST} & \multicolumn{2}{c|}{BreastMNIST} & \multicolumn{2}{c}{DermaMNIST} \\
%          & AUC$\uparrow$ & ACC$\uparrow$ & AUC$\uparrow$ & ACC$\uparrow$ & AUC$\uparrow$ & ACC$\uparrow$ \\
%         \toprule
%         MedMNIST Benchmark & \textbf{99.10} & 94.60 & 91.90 & 86.30 & 92.00 & 76.80 \\
%         DWT-CV \cite{cheng2022dwt} & 95.69 & 88.67 & 89.77 & 85.68 & 91.67 & 74.75 \\ 
%         SADAE \cite{ge2022self} & 98.30 & 91.80 & 91.50 & 87.80 & 92.70 & 75.90 \\
%         \midrule
%         ROCO(LP) & 89.20 & 81.57 & 78.85 & 71.47 & 87.28 & 64.69 \\
%         MedICaT(LP) &  \\
%         PMC OA(LP) & 93.35 & 85.50 & 88.41 & 79.49 & 90.81 & 71.97 \\
%         \midrule
%         ROCO(FT) & 98.78 & 93.99 & 94.42 & 90.06 & 91.11 & 78.65 \\
%         MedICaT(FT) &  \\
%         Ours(FT) & 99.02 & \textbf{95.35} & \textbf{94.56} & \textbf{91.35} & \textbf{93.41} & \textbf{79.80} \\
%         \midrule
%     \end{tabular}
%     \caption{MedMNIST, LP: LinearProbe; FT: FineTune}
%     \label{tab:MedMNIST}
% \end{table*}
% 
% =============================================================================


==> content/tab/dataset_statistic.tex <==
\begin{table}[]
\setlength\tabcolsep{8pt}
\centering
\caption{Dataset Statistics. "Medical" refers to the data filtered by the image classification and keyword filtering.}
\begin{tabular}{lll}
\hline
Dataset Statistic             & Number                & Ratio            \\ \hline
Figures                       & 12,211,907            & 100\%            \\
Medical Figures               & 381,096               & 3.12\%           \\
Medical Figure w. Subfigures  & 378,717               & 3.1\%            \\
Medical Figure w. Subcaptions & 239,905               & 1.96\%           \\
Medical Figure w. Both        & 239,905               & 1.96\%           \\
Subfigures                    & 1,848,729             & 100\%            \\
Medical Subfigures            & 1,646,592             & 89.07\%          \\
Subcaptions                   & 898,467             & 100\%            \\
Avg. Subcaption Tokens        & 32.4                & \-            \\
Subfigure-Subcaption Pairs    & 36,060$\sim$1,003,911 & 2.2\%$\sim$61.0\% \\ \hline
\end{tabular}

\end{table}




==> content/tab/medmnist.tex <==
% 
% MedMNIST 的所有 subset 结果
% 
\begin{table*}[htpb]
    \centering
    \setlength{\tabcolsep}{6pt} % Default value: 6pt
    % \renewcommand{\arraystretch}{1.5} % Default value: 1
    \caption{Full results on MedMNIST. Only 3/12 are shown in main text}
    \begin{tabular}{l|cc|cc|cc}
    \toprule
        % Modality & Chest X-Ray & Ultrasound	& Dermatoscope \\
        Dataset & \multicolumn{2}{c|}{PneumoniaMNIST} & \multicolumn{2}{c|}{BreastMNIST} & \multicolumn{2}{c}{DermaMNIST} \\
        Method & AUC$\uparrow$ & ACC$\uparrow$ & AUC$\uparrow$ & ACC$\uparrow$ & AUC$\uparrow$ & ACC$\uparrow$ \\
        \toprule
        ResNet50 & 96.20 & 88.40 & \cellcolor{lightergray}91.90 & 86.60 & 91.20 & 73.10 \\
        % Benchmark & \textbf{99.10} & 94.60 & 91.90 & 86.30 & 92.00 & 76.80 \\
        DWT-CV \cite{cheng2022dwt} & 95.69 & 88.67 & 89.77 & 85.68 & 91.67 & 74.75 \\ 
        SADAE \cite{ge2022self} & \cellcolor{lightergray}98.30 & \cellcolor{lightergray}91.80 & 91.50 & \cellcolor{lightergray}87.80 & \cellcolor{lightergray}92.70 & \cellcolor{lightergray}75.90 \\
        \midrule
        % PMC OA(LP) & 93.35 & 85.50 & 88.41 & 79.49 & 90.81 & 71.97 \\
        BioMed-CLIP & \cellcolor{lightgray} 99.02 & \cellcolor{lightgray}95.35 & \cellcolor{lightgray}94.56 & \cellcolor{lightgray}91.35 & \cellcolor{lightgray}93.41 & \cellcolor{lightgray}79.80 \\
     \bottomrule
    \end{tabular}
    \label{tab:MedMNIST_Appendix}
\end{table*}



==> content/tab/retrieval_1.tex <==
\begin{table*}[t]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{4pt} % Default value: 6pt
    % \renewcommand{\arraystretch}{1.5} % Default value: 1
    \begin{tabular}{lcc|ccc|ccc}
        \multirow{2}{*}{Methods} & \multirow{2}{*}{Pretrain Data} & \multirow{2}{*}{DataSize} & \multicolumn{3}{c|}{I2T} & \multicolumn{3}{c}{T2I} \\
        ~ & ~ & ~ & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 \\
        \toprule
        M3AE \cite{chen2022multi} & \scriptsize ROCO, MedICaT & 233 K & 19.10 & 45.60 & 61.20 & 19.05 & 47.75 & 61.35 \\
        ARL \cite{chen2022align} & \scriptsize ROCO, MedICaT, MIMIC-CXR & 233 K & 23.45 & 50.60 & 62.05 & 23.50 & 49.05 & 63.00 \\
        \midrule
        MedCLIP-RN50 & \scriptsize ROCO & 60 K & 22.83 & 50.60 & 60.58 & 21.82 & 49.34 & 60.94 \\
        MedCLIP-RN50x4 & \scriptsize ROCO & 60 K & 24.34 & 52.27 & 64.42 & 22.98 & 50.60 & 64.77 \\
        MedCLIP-RN50x8 & \scriptsize ROCO & 60 K & 26.01 & 54.13 & 65.27 & 25.05 & 52.82 & 64.01 \\
        MedCLIP-RN50x16  & \scriptsize ROCO & 60 K & 23.74 & 54.33 & 67.49 & 24.80 & 54.49 & 67.24 \\ 
        \midrule
        % MedCLIP-RN50  & \scriptsize ROCO, MedICaT & 233 K & 29.28 & \textbf{59.88} & \textbf{71.42} & \textbf{28.23} & \textbf{58.06} & \textbf{69.56} \\
        % MedCLIP-RN50  & \scriptsize ROCO, MedICaT, MIMIC-CXR, PMC OA & 1.6 M \\
        % \midrule
        MedCLIP-RN50 & \scriptsize MedICaT & 173 K & 12.30 & 35.28 & 46.52 & 13.36 & 35.84 & 47.38 \\
        MedCLIP-RN50 & \scriptsize PMC OA & 1.6 M & \textbf{30.42} & 59.11 & 70.16 & 27.92 & 55.99 & 66.35 \\
        MedCLIP-RN50 & \scriptsize Denoised PMC OA & 1.6 M &   \\
        \midrule
    \end{tabular}
    \caption{Zero-shot on ROCO Test}
    \label{tab:Zeroshot-ROCO}
\end{table*}

\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{6pt} % Default value: 6pt
    % \renewcommand{\arraystretch}{1.5} % Default value: 1
    \begin{tabular}{ll|ccc|ccc}
        \multirow{2}{*}{Methods} & \multirow{2}{*}{Extra Data} & \multicolumn{3}{c|}{I2T} & \multicolumn{3}{c}{T2I} \\
        ~ & ~ & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 \\
        \toprule
        M3AE \cite{chen2022multi} & MedICaT & 22.90 & 51.05 & 65.80 & 22.20 & 52.50 & 66.65 \\
        ARL \cite{chen2022align} & MedICaT + MIMIC-CXR & 29.35 & 57.50 & 70.40 & 29.65 & 56.95 & 69.30 \\
        \midrule
        MedCLIP-RN50 & \usym{2717} & 22.83 & 50.60 & 60.58 & 21.82 & 49.34 & 60.94 \\
        MedCLIP-RN50x4 & \usym{2717} & 24.34 & 52.27 & 64.42 & 22.98 & 50.60 & 64.77 \\
        MedCLIP-RN50x8 & \usym{2717} & 26.01 & 54.13 & 65.27 & 25.05 & 52.82 & 64.01 \\
        MedCLIP-RN50x16  & \usym{2717} & 23.74 & 54.33 & 67.49 & 24.80 & 54.49 & 67.24 \\ 
        \midrule
        MedCLIP-RN50  & MedICaT & \\ 
        MedCLIP-RN50x4 & MedICaT & \\
        \midrule
        MedCLIP-RN50(ZS) & PMC OA & 30.42 & 59.11 & 70.16 & 27.92 & 55.99 & 66.35 \\
        MedCLIP-RN50 & PMC OA & \textbf{36.51} & \textbf{69.43} & \textbf{80.05} & \textbf{36.51} & \textbf{68.54} & \textbf{79.17} \\
        MedCLIP-RN50 & Denoised PMC OA &  \\
        % MedCLIP-RN50x4 & PMC OA & \\
        % MedCLIP-RN50x16  & PMC OA & \\ 
        \midrule
    \end{tabular}
    \caption{Fine-tune on ROCO Test}
    \label{tab:Finetune-ROCO}
\end{table*}

